Human mobility networks reveal increased segregation in large cities

A long-standing expectation is that large, dense, and cosmopolitan areas support socioeconomic mixing and exposure between diverse individuals. It has been difficult to assess this hypothesis because past approaches to measuring socioeconomic mixing have relied on static residential housing data rather than real-life exposures between people at work, in places of leisure, and in home neighborhoods. Here we develop a new measure of exposure segregation (ES) that captures the socioeconomic diversity of everyday encounters. Leveraging cell phone mobility data to represent 1.6 billion exposures among 9.6 million people in the United States, we measure exposure segregation across 382 Metropolitan Statistical Areas (MSAs) and 2829 counties. We discover that exposure segregation is 67% higher in the 10 largest Metropolitan Statistical Areas (MSAs) than in small MSAs with fewer than 100,000 residents. This means that, contrary to expectation, residents of large cosmopolitan areas have significantly less exposure to diverse individuals. Second, we find evidence that large cities offer a greater choice of differentiated spaces targeted to specific socioeconomic groups, a dynamic that accounts for this increase in everyday socioeconomic segregation. Third, we discover that this segregation-increasing effect is countered when a city's hubs (e.g. shopping malls) are positioned to bridge diverse neighborhoods and thus attract people of all socioeconomic statuses. Overall, our findings challenge a long-standing conjecture in human geography and urban design, and highlight how built environment can both prevent and facilitate exposure between diverse individuals.

==> 02-main_figures.tex <==











  


















==> deprecated_content.tex <==




\begin{figure}[htbp]
  \centering
  \begin{subfigure}{0.4\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figures/fig2_ucurve_a.pdf}
  \caption{}
\end{subfigure}
  \begin{subfigure}{0.4\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figures/fig2_ucurve_b.pdf}
  \caption{}
\end{subfigure}
  \caption{\textbf{The highest and lowest ES deciles are especially isolated.}\\
  For each MSA we plot the ratio of actual path crossings within each ES decile to the expected number of path crossings under a null model in which people crossed paths uniformly at random: for example, a ratio of 2 indicates that there are twice as many within-decile path crossings as would be expected if there were uniform interaction between deciles. %
  Ratios for all ES deciles are greater than one, indicating that people are disproportionately likely to cross paths with those in their own ES decile. This trend is especially pronounced for the highest and lowest ES deciles, as indicated by the U-shaped curves. The solid line indicates the median ratio across MSAs, and the shaded region indicates the 10\% to 90\% percentiles across MSAs. \textbf{(a)} shows results for all path crossings, and \textbf{(b)} stratifies by by whether path crossings occur at leisure, work, or home locations. Home path crossings are particularly likely to be within-decile. Home path crossings are those where both people are in their home Census tract; work path crossings occur when both people are at their inferred work location; and leisure path crossings are those which occur at any category in the ``Leisure'' category, as defined in Methods. Supplementary Figure \ref{fig:decile_heatmap} plots the ratios for all pairs of ES deciles.\emma{Note that what is being plotted here is NOT the same as the interaction segregation measure. We discussed this and decided that it did not make sense to use interaction segregation here. However, we agree it is slightly confusing. One option might be to move Figure 2 to Figure 4, so we don't switch away from our interaction segregation measure immediately after we've introduced it.}
}
    \label{fig:main_4}
\end{figure}


\begin{figure}[htbp]
\centering
\begin{subfigure}[t]{.4\textwidth}
  \includegraphics[width=\textwidth,keepaspectratio]{figures/segregation_by_hour.pdf}
   \caption{}
\end{subfigure}
\begin{subfigure}[t]{.4\textwidth}
  \includegraphics[width=\textwidth,keepaspectratio]{figures/feature_type_rainbow_rent_zestimate.pdf}
  \caption{}
\end{subfigure}
\caption{\textbf{Segregation varies by time and function.} \textbf{(a)} Interaction segregation varies over the course of the day. The vertical axis plots interaction segregation for each Metropolitan Statistical Area (MSA) during the local time intervals indicated on the horizontal axis. The shaded region indicates the 10\% to 90\% percentile across MSAs for each time bucket. The black line represents the median segregation over all MSAs. Median segregation is  higher at night (0.46 from 9PM-12AM) when more people are in their home Census tract, and lower during the day (0.36 from 9AM-12PM).
\textbf{(b)} Interaction segregation varies by function. Each point represents interaction segregation in one MSA using only path crossings which occur in a given place (Methods); the boxes indicate the interquartile range across MSAs. Places are divided into home, work, transportation, and leisure. The vertical line indicates the median overall segregation across MSAs. Segregation is highest when both people are in their home tract, and lower for work, transportation, and leisure path crossings. Segregation varies by leisure category, and is 3x higher in golf courses (the most segregated category) than in stadiums (the least segregated category) \wl{32\% absolute / 195\% relative} \emma{wenli, can you confirm that my 3x is correct?}
}
 \label{fig:main_3}
\end{figure}


\paragraph{Segregation by SES decile.} 

Having established that interaction segregation is smaller than NSI, we search for settings in which higher levels of segregation nonetheless emerge using our more realistic measure. We first assess how segregation varies across SES deciles, defining the segregation of each decile as the ratio of observed interactions within each SES decile to the expected number of interactions if people crossed paths uniformly at random (Methods). Higher ratios indicate that people are more likely to cross paths with those in the same SES decile, indicating higher levels of segregation.\emma{Does the switch in Figure 2 to observed:expected interactions make sense (is it necessary)? What is the succinct justification for the change? I think it's that we're comparing the relative segregation of groups of people, as opposed to groups of interactions, but think about how to express this succinctly.} \blanca{Are you asking why we shift to using a ratio of edges in fig2 vs actual segregation differences between the deciles? My understanding--please correct me if I'm wrong or misunderstood your comment--is that here we're measuring the strength of the ties between deciles (so we are computing a function of the number of ties between discrete groups of people rather than a function of the difference in their SES)} As Figure \ref{fig:main_2}a illustrates, while ratios for all deciles exceed one, segregation is highest in the top and bottom deciles. In Figure \ref{fig:main_2}a, we show that this relationship persists across home, work, and leisure interactions, and that segregation is particularly high for home interactions, consistent with Figure \ref{fig:main_1}. (Home interactions are defined as those where both people are in their home Census tract; work path as those where both people are at their inferred work location, as defined in the Methods; and leisure interactions are those which occur at any category in the ``Leisure'' category, as defined in Methods.)

\emma{Not mentioning Figure \ref{fig:louvain} at present - I feel like it just gives us more work to do without adding much to the main story, so would lean towards cutting.} 



\paragraph{Segregation by time of day}

We next assess whether there are times of day associated with particularly high levels of segregation (Figure \ref{fig:main_3} by applying our mixed model to interactions which occur at varying times of day (eg, 6 AM-9 AM local time versus 6 PM - 9 PM local time). We find that is highest at night, when a larger proportion of people are at home, consistent with the fact that segregation is highest in residential areas. 

\begin{figure}[htbp]
  \includegraphics[width=\textwidth,height=\textheight,keepaspectratio, trim=2 2 2 2,clip]{figures/descriptive_statistics_census}
  \caption{\textbf{Descriptive statistics of path crossings 2.}\\
  (a) xxx. \\
  (b) xxx. \\
  (c) xxx. \\
  (d) xxx.}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth, keepaspectratio]{figures/top10_heatmaps.pdf}
  \caption{\textbf{Within-decile interactions are enriched in the top 10 MSAs, while between-decile interactions are lower than expected.}
  For each MSA we plot the ratio of actual path crossings of each ES decile to the expected number of path crossings; see Figure~\ref{fig:main_2} and \ref{sec:methods}. The diagonal entries of each heatmap correspond to the within-decile ratio of actual:expected interactions, while the off-diagonal entries correspond to the between-decile ratio of actual:expected interactions. A higher number indicates a higher level of interaction.
  }
  \label{fig:decile_heatmap}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[height=5in,keepaspectratio]{figures/boxplot-neighborhood.png}
\caption{Neighborhood detection from path crossing data. \\
For each of the 10 most populous MSAs, we compute a graph where nodes are Census tracts and the edge weight between two nodes represents the ratio of observed to expected path crossings between residents of those Census tracts. Higher edge weights capture pairs of neighborhoods whose residents cross paths more than expected. We then apply the Louvain clustering algorithm to the graph to extract neighborhoods for each MSA's most populous principal city. (Top) The neighborhoods discovered by our clustering algorithm (left panel) trace racial and socioeconomic boundaries (right three panels indicate \% Black, \% white, and median household income) despite the fact that no demographic information was used in the clustering. We plot maps of Washington DC to highlight this result. (Bottom) We can quantify this effect more systematically by comparing demographic differences between pairs of adjacent census tracts within each city depending on whether they are in the \emph{same} neighborhood (blue bars) or \emph{different} neighborhoods (red bars). Across cities, red bars are right-shifted relative to blue bars, indicating that adjacent Census tracts that lie in different neighborhoods are more demographically different than those that lie in the same neighborhood. This indicates that our clustering algorithm is recovering demographic boundaries within each city.}
\label{fig:louvain}
\end{figure}
